Alternating Arm Exponents for the Critical Planar Ising Model

We derive the alternating arm exponents of critical Ising model. We obtain six different patterns of alternating boundary arm exponents which correspond to the boundary conditions $(\ominus\oplus)$, $(\ominus\text{free})$ and $(\text{free}\text{free})$, and the alternating interior arm exponents.

==> tex/ising_interior.tex <==
\begin{figure}[ht!]
\begin{subfigure}[b]{0.5\textwidth}
\begin{center}
\includegraphics[width=\textwidth]{figures/ising_interior_ws}
\end{center}
\caption{$\LA^{I/I}(n,N)$ is the well-separated arm event. }
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
\begin{center}\includegraphics[width=\textwidth]{figures/ising_interior_interface}
\end{center}
\caption{The four gray parts are $R_1$ to $R_4$ respectively. }
\end{subfigure}
\caption{\label{fig::ising_interior} The explanation of the proof of Theorem \ref{thm::ising_interior}.}
\end{figure}

\begin{proof}[Proof of Theorem \ref{thm::ising_interior}]
We only give the proof for $\alpha_4$ and the other cases can be proved similarly. Consider $\Lambda_m$ with two boundary points $a_m=(-m,0)$ and $b_m=(m,0)$. Fix the $(\ominus\oplus)$ boundary condition: the vertices along $\partial\Lambda_m$ from $b_m$ to $a_m$ (counterclockwise) are $\oplus$ and the vertices from $a_m$ to $b_m$ are $\ominus$. Since we fix $\beta=\beta_c$ and the boundary conditions, and $\omega=(1010)$, we eliminate them from the notations. We will prove that, for $n<N\le m/2$, 
\begin{equation}\label{eqn::ising_4arms}
\mu_{\Lambda_m}[\LA(n,N)]=N^{-\alpha_4+o(1)},\quad \text{as }N\to \infty.
\end{equation}

Fix the landing sequence $I=(I_1, I_2, I_3, I_4)$ where 
\[I_1=[-1/2, 1/2]\times\{-1\}, \quad I_2=\{-1\}\times [-1/2, 1/2],\quad I_3=[-1/2, 1/2]\times\{1\},\quad I_4=\{1\}\times [-1/2, 1/2].\] 
Recall that $\LA^{I/I}(n,N)$ is the $1/8$-well-separated arm events with the landing sequence $nI$ on $\partial \Lambda_n$ and $NI$ on $\Lambda_N$. The four arms in $\LA(n,N)$ are denoted by $(\gamma_1, \gamma_2, \gamma_3, \gamma_4)$ where $\gamma_1$ and $\gamma_3$ are $\oplus$ and $\gamma_2$ and $\gamma_4$ are $\ominus$. 

Consider critical Ising model in $\Lambda_{2N}$. Let $R_1$ to be the rectangle $[-3N/4, 3N/4]\times [-2N, -N]$, and define $\LC^{\oplus}_1$ to be the event that $\gamma_1$ is connected by path of $\oplus$ in $R_1$ to the bottom of $R_1$. Let $R_2$ to be the rectangle $[-9N/8, -N]\times[-N/2,2N]$, and define $\LC_2^{\ominus}$  to be the event that $\gamma_2$ is connected by path of $\ominus$ in $R_2$ to the top of $R_2$. Let $R_3$ be the rectangle $[-3n/4, 3n/4]\times[-n,n]$, and define $\LC_3^{\oplus}$ to be the event that $\gamma_3$ is connected to $\gamma_1$ by path of $\oplus$ in $R_3$. Let $R_4$ be the rectangle $[N, 9N/8]\times[-N/2,2N]$, and define $\LC_4^{\ominus}$ to be the event that $\gamma_4$ is connected by path of $\ominus$ in $R_4$ to the top of $R_4$. See Figure \ref{fig::ising_interior}.

By (\ref{eqn::ising_boundary_comparison}), Propositions \ref{prop::ising_rsw} and \ref{cor::ising_spacemixing}, we could prove
\begin{equation}\label{eqn::ising_interior_aux1}
\mu_{\Lambda_{2N}}\left[\LA^{I/I}(n,N)\right]\asymp \mu_{\Lambda_{2N}}\left[\LA^{I/I}(n,N)\cap\LC^{\oplus}_1\cap\LC_2^{\ominus}\cap\LC^{\oplus}_3\cap\LC^{\ominus}_4\right],
\end{equation}
where the constants in $\asymp$ are uniform over $n,N$. 

Let $\PP_N$ be the probability measure $\mu_{\Lambda_{2N}}$ where the square lattice is scaled by $1/N$ and let $\PP_{\infty}$ be the law of $\SLE_{3}$ in $[-2,2]\times[-2,2]$ from $(-2,0)$ to $(2,0)$. On the event $\LA^{I/I}(n,N)\cap\LC^{\oplus}_1\cap\LC_2^{\ominus}\cap\LC^{\oplus}_3\cap\LC^{\ominus}_4$, consider the interface $\eta$ from $a_{2N}$ to $b_{2N}$. Let $\tau_1$ be the first time that $\eta$ hits $\partial\Lambda_n$. The event $\LC_1^{\oplus}\cap\LC_2^{\ominus}$ guarantees that $\eta[0,\tau_1]$ is bounded away from the target $b_{2N}$. The event $\LC^{\oplus}_3$ guarantees that, after $\tau_1$, the path $\eta$ hits the neighborhood of $(0,2N)$ at some time $\sigma_1$. The event $\LC^{\ominus}_4$ guarantees that, after $\sigma_1$, the path $\eta$ hits $\partial\Lambda_n$ again. Therefore, for $\eps>0$, we have
\[\limsup_{N\to \infty}\PP_N\left[\LA^{I/I}(\eps N,N)\cap\LC^{\oplus}_1\cap\LC_2^{\ominus}\cap\LC^{\oplus}_3\cap\LC^{\ominus}_4\right]\le \eps^{\alpha_4+o(1)}\le\liminf_{N\to\infty}\PP_{N}[\LA(\eps N, N)].\]
Combining with Lemma \ref{lem::wellseparated_comparable} and (\ref{eqn::ising_interior_aux1}), we have 
\[\liminf_{N\to\infty}\PP_{N}[\LA(\eps N, N)]\asymp \limsup_{N\to\infty}\PP_{N}[\LA(\eps N, N)]\asymp \eps^{\alpha_4+o(1)}.\]
By Corollary \ref{cor::ising_spacemixing}, we know that 
\begin{equation}\label{eqn::ising_interior_aux2}
\liminf_{N\to \infty}\mu_{\Lambda_m}\left[\LA(\eps N, N)\right]\asymp \limsup_{N\to\infty}\mu_{\Lambda_m}\left[\LA(\eps N, N)\right]\asymp \eps^{\alpha_4+o(1)},
\end{equation} 
where the constants in $\asymp$ are uniform over $\eps$ and $m\ge 2N$. 

Suppose $N=n\eps^{-K}$ for some integer $K$. By Proposition \ref{prop::qm_interior_alternating}, for $m\ge 2N$, we have 
\[\mu_{\Lambda_m}\left[\LA(n, N)\right]\le C^K\Pi_{j=1}^K\mu_{\Lambda_m}\left[\LA(n\eps^{-j+1}, n\eps^{-j})\right],\]
where $C$ is some universal constant. Thus
\[\frac{\log\mu_{\Lambda_m}\left[\LA(n, N)\right]}{\log N}\le \frac{K\log C}{\log N}+\frac{1}{\log N}\sum_{j=1}^K\log \mu_{\Lambda_m}\left[\LA(n\eps^{-j-1}, n\eps^{-j})\right].\]
By (\ref{eqn::ising_interior_aux2}), we have 
\[\limsup_{j\to \infty}\mu_{\Lambda_m}\left[\LA(n\eps^{-j-1}, n\eps^{-j})\right]\asymp \eps^{\alpha_4+o(1)}.\]
Therefore,
\[\limsup_{K\to \infty}\frac{\log\mu_{\Lambda_m}\left[\LA(n, N)\right]}{\log N}\le\frac{\tilde{C}}{\log(1/\eps)}-\alpha_4,\]
where $\tilde{C}$ is some universal constant. Let $\eps\to 0$, we have 
\[\limsup_{N\to \infty}\frac{\log\mu_{\Lambda_m}\left[\LA(n, N)\right]}{\log N}\le-\alpha_4.\]
We could prove the lower bound similarly:
\[\liminf_{N\to \infty}\frac{\log\mu_{\Lambda_m}\left[\LA(n, N)\right]}{\log N}\ge -\alpha_4.\]
These imply (\ref{eqn::ising_4arms}) and complete the proof. 
\end{proof}
















 

